Not All GPUs Are Created Equal: Characterizing Variability in Large-Scale, Accelerator-Rich Systems

Scientists are increasingly exploring and utilizing the massive parallelism of general-purpose accelerators such as GPUs for scientific breakthroughs. As a result, datacenters, hyperscalers, national computing centers, and supercomputers have procured hardware to support this evolving application paradigm. These systems contain hundreds to tens of thousands of accelerators, enabling peta- and exa-scale levels of compute for scientific workloads. Recent work demonstrated that power management (PM) can impact application performance in CPU-based HPC systems, even when machines have the same architecture and SKU (stock keeping unit). This variation occurs due to manufacturing variability and the chip's PM. However, while modern HPC systems widely employ accelerators such as GPUs, it is unclear how much this variability affects applications. Accordingly, we seek to characterize the extent of variation due to GPU PM in modern HPC and supercomputing systems. We study a variety of applications that stress different GPU components on five large-scale computing centers with modern GPUs: Oak Ridge's Summit, Sandia's Vortex, TACC's Frontera and Longhorn, and Livermore's Corona. These clusters use a variety of cooling methods and GPU vendors. In total, we collect over 18,800 hours of data across more than 90% of the GPUs in these clusters. Regardless of the application, cluster, GPU vendor, and cooling method, our results show significant variation: 8% (max 22%) average performance variation even though the GPU architecture and vendor SKU are identical within each cluster, with outliers up to 1.5X slower than the median GPU. These results highlight the difficulty in efficiently using existing GPU clusters for modern HPC and scientific workloads, and the need to embrace variability in future accelerator-based systems.

==> future.tex <==
\section{Next Steps}
\label{sec:future}

\begin{enumerate}
  \item Our current study was done using only one kind of application (a SGEMM kernel). A natural next step is to repeat the study with additional benchmarks that stress different GPU components. This will also help us determine which kind of applications are more susceptible to being affected by performance variation. In particular, we plan on using some of the CORAL-2 benchmarks~\cite{coral2} to extend our study across benchmarks that stress a variety of GPU components.

  \item We plan to repeat our study on NVIDIA V100 GPUs on AMD MI50 and MI60 GPUs in some of the national lab clusters, to determine if this problem exists across vendors.

  \item Finally, since users have a high likelihood of being allocated GPUs with variable performance, it is important to develop application-level strategies to mitigate the effects of performance variation and make power management a first-class citizen in future accelerator-driven, exascale systems~\cite{SinclairVenkataraman2021-ascr}.
\end{enumerate}


==> results-cloudlab.tex <==
\section{CloudLab} %
\label{sec:res-cloudlab}

\begin{figure*}[tb!]
  \centering
  \includegraphics[width=0.24\textwidth]{figures/cloudlab-plots/cloudlab-no-breakdown-pwr.pdf}
  \includegraphics[width=0.24\textwidth]{figures/cloudlab-plots/cloudlab-no-breakdown-freq.pdf}
  \includegraphics[width=0.24\textwidth]{figures/cloudlab-plots/cloudlab-no-breakdown-temp.pdf}
  \includegraphics[width=0.24\textwidth]{figures/cloudlab-plots/cloudlab-no-breakdown-perf.pdf}
  \vspace{-0.3cm}
  \caption{Summary results from CloudLab, showing variation in performance (kernel duration), measured frequency, power and temperature as reported by NVIDIA's profiler, when running the GPUs unthrottled at the TDP value of 300W. For performance (SGEMM kernel duration) lower times are better. For frequency higher values are better.}
  \label{fig:cloudlab-summary}
\end{figure*}

Figure~\ref{fig:cloudlab-summary} shows how the SGEMM kernel performs on CloudLab, with box plots for kernel duration, SM frequency, power, and temperature data aggregated from multiple runs over a week.
These aggregated plots help us identify trends across the GPUs.
Overall, we observe up to a 5\% difference in performance (kernel duration) overall for the SGEMM kernel.
Further from Figure~\ref{fig:cloudlab-summary} we can see that the temperatures for these 12 GPUs are tightly packed tightly (4\degree C between $Q1$ and $Q3$), and the measured frequencies have a wider spread (60 MHz, 5\% difference, between $Q1$ and $Q3$) like the kernel duration.
Despite pinning the GPU frequency to the highest (1530 MHz), and enforcing the highest power limit (300W), the data shows GPUs operating at lower frequency.

\begin{figure*}[tb!]
  \centering
  \begin{subfigure}{0.9\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/cloudlab-plots/cloudlab-pwr-timeline-gpu-0-4.pdf}
    \caption{Power}
    \label{fig:cloudlab-pwr-timeline}
  \end{subfigure}
  \begin{subfigure}{0.9\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/cloudlab-plots/cloudlab-freq-timeline-gpu-0-4.pdf}
    \caption{Frequency}
    \label{fig:cloudlab-freq-timeline}
  \end{subfigure}
  \vspace{-0.3cm}
  \caption{Time-series plots for frequency and power for two distinct GPUs executing the SGEMM Kernel.}
  \label{fig:cloudlab-timelines}
\end{figure*}

Prior work on GPUs, indicates that these changes in frequency could have been caused by intervention from the PM infrastructure~\cite{GeVogt2013-dvfsKepler}.
To investigate this, we created time-series view of the changes in frequency and power drawn for the SGEMM kernel as observed in our experiments. We present these views in Figure~\ref{fig:cloudlab-timelines}.
The vertical tabs indicate the start time of a new kernel, at this point the GPU reports to be running at the last observed frequency (1327 MHz, for GPU-0).
As the kernel begins executing, the frequency starts to rise along with an increase in power drawn.
As the frequency approaches 1357 MHz (highest observed for GPU-0), the power reaches and exceeds the 300W limit.
This can be seen in the power vs time plot of the Figure~\ref{fig:cloudlab-timelines}.
At this point the frequency of the GPU starts to drop and, in a few time-steps stabilizes, then stays at this level till the end of the kernel execution.
We see a similar trend for GPU-1 presented using orange color in Figure~\ref{fig:cloudlab-timelines}.
Thus, we can see that changes in frequency are correlated with power changes.

\begin{figure*}[tb!]
  \centering
  \begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/cloudlab-plots/cloudlab-perf-freq-scatterplot.pdf}
    \caption{Kernel Duration vs. Frequency}
    \label{fig:cloudlab-perf-freq}
  \end{subfigure}
  \hspace{6ex}
  \begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/cloudlab-plots/cloudlab-perf-temp-scatterplot.pdf}
    \caption{Kernel Duration vs. Temperature}
    \label{fig:cloudlab-perf-temp}
  \end{subfigure}
  \vspace{-0.3cm}
  \caption{Possible correlations between performance, temperature, and measured frequency for SGEMM kernel among CloudLab.}
  \label{fig:cloudlab-scatterplots}
\end{figure*}

Prior work in CPUs shows that changes in frequencies lead to the performance variation~\cite{chasapis2016runtime, ChasapisMoreto2019-powerEfficJobSched, DasOzdemir2007-processVar, InadomiPatki2015-scVar, v100-tc}. The results from Figure~\ref{fig:cloudlab-timelines} and Figure~\ref{fig:cloudlab-scatterplots} indicate that similar variations may exist in GPUs, to further investigate, we take a closer look at the differences between performance, frequency, and temperature in Figure~\ref{fig:cloudlab-scatterplots}.
In Figure~\ref{fig:cloudlab-scatterplots} we can observe that when frequency increases kernel performance improves (i.e., kernel duration decreases).
For example, GPU-9 runs at 1297 MHz with kernel duration of 2550 ms compared to GPU-10 running at 1350MHz has a kernel duration of 2460 ms.
This indicates that SGEMM has smaller kernel durations (better performance) at higher frequencies.

In Figure~\ref{fig:cloudlab-scatterplots}, we observe the recorded temperatures are clustered together within a tight band (4\degree C).
Hence, we cannot make any substantial claims about thermal effects based on this data.
Interestingly %
multiple GPUs run at the same temperature but obtain very different performance.
For example, GPU-7 and GPU-0 have a 50 ms difference in kernel durations while running at the same temperature (69\degree C).
Thus, we observe GPUs having both good and bad performance while running at the same temperature.

More broadly, these results indicate that similar GPUs could have performance variation by up to 5\%, even when the user pins the GPU to the maximum frequency and power limit.
To validate this trend, we collect data from more GPUs in a larger cluster. 


==> results-implications.tex <==
\subsection{Real World Implications}
\label{sec:res-impl}

To understand the real-world implications of the observed performance variation we need to understand how it would affect users across multiple allocation requests, including for either one GPU or multiple GPUs.  

\subsubsection{Single GPU Experiments}
\label{subsubsec:res-impl-singleGPU}

Of the 388 GPUs we collected measurements from in Longhorn, 71 GPUs are 6-7\% (or about 150 ms) slower than the fastest GPUs in the cluster.
Thus, users running single GPU experiments on Longhorn would have an 18\% chance of being assigned a slower GPU.
Additionally, we also observed that individual GPUs in Longhorn had some degree of performance variation (ranging from 1\% on average, up to 14\%) among themselves between different runs.
Similarly, in Vortex 18 of the 184 GPUs are 6-7\% (or about 150ms) slower than the fastest observed GPUs in the cluster.
Thus, a user running a single GPU experiment on Vortex has a 10\% chance of being assigned a slower GPU.
Finally, in Summit, of the 26,802 GPUs we observed, 2,490 GPUs are 6-7\% (or about 160 ms) slower than the fastest GPUs in the supercomputer.
Like Longhorn, Summit also has variance within specific GPUs (Section~\ref{subsubsec:res-summit-rowh}).
Thus, a user running a single GPU experiment on Summit has a 9\% chance of being assigned a slower GPU.
Overall, this performance variation could significantly affect any claims they make about their applications performance.

\subsubsection{Multiple GPU Experiments}
\label{subsubsec:res-impl-multiGPU}

If a user is running multi-GPU experiments, they are even more likely to be assigned a slower GPU.
For example, if a user requests 4 GPUs on Longhorn, 40\% (40/104) to 50\% (53/104) percent of the time they will be assigned a slower GPU.\footnote{There is a range because 18 of the GPUs did not provide sufficient information for us to identify the node info.  Since we were able to identify 35 nodes, in the worst case these 18 additional GPUs are spread across 18 additional nodes and in the best case they would be spread across 5 additional nodes.}
Similarly, for Vortex, a user requesting 4 GPUs will get a slow GPU 22\% - 25\% of the time, and for Summit a user requesting 4 GPUs will get a slow GPU 37\% of the time. 
Thus, from a user’s perspective, they are likely to get a slow GPU frequently.
This makes it imperative for cluster operators to identify and mitigate these issues. 

From an operator’s perspective, the information in this study can be used to improve the operation of the cluster, and more specifically help develop strategies for better maintenance.
The study methodology helps in identifying problem nodes that have clearly underperforming GPUs and perform targeted maintenance on them.
Performance variation may be application dependent, in the current study we only focused on a particular kind kernel.
We plan to run experiments with different kinds of applications to improve our understanding of performance variation.
Finally, we envision the need to develop strategies for cluster operations, like cooling and node allocation, to help mitigate the effects of performance variation.


==> results-ornl-dayOfWeek.tex <==
\subsubsection{Day of Week Results}
\label{subsubsec:res-summit-dayOfWeek}

\begin{figure*}[tb!]
  \centering
  \begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/summit-plots/sgemm-summit-perf-weekday-breakdown.pdf}
    \caption{Performance}
    \label{fig:summit-weekday-perf}
  \end{subfigure}
  \begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/summit-plots/sgemm-summit-freq-weekday-breakdown.pdf}
    \caption{Frequency}
    \label{fig:summit-weekday-freq}
  \end{subfigure}
  \begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/summit-plots/sgemm-summit-pwr-weekday-breakdown.pdf}
    \caption{Power}
    \label{fig:summit-weekday-pwr}
  \end{subfigure}
  \begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/summit-plots/sgemm-summit-temp-weekday-breakdown.pdf}
    \caption{Temperature}
    \label{fig:summit-weekday-temp}
  \end{subfigure}
  \vspace{-0.3cm}
  \caption{Day of the week summary results for Summit. We see more outliers in frequency, power, and temperature on Mondays, Wednesdays, and Fridays.}
  \label{fig:summit-weekday-summary}
  \vspace{-1ex}
\end{figure*}

Similar to TACC, we study how variation across GPUs behaves over time by bucketing the data
according to the day of the week in Figure~\ref{fig:summit-weekday-summary}.
As mentioned in Section~\ref{sec:method}, our data from Summit is aggregated over eight weeks, and subdivided by the day of the week it was collected on.
Similar to TACC, we observe an overall consistent trend in variation across each day of the week, being around 8\%.
However, unlike TACC, there are no days that stand out as an anomaly, potentially because we
collected a more consistent number of samples throughout the week. %
Nevertheless, we observe a higher concentration of GPUs which consume below 290W on Monday, Wednesday, and Friday.
Surprisingly, even with more power outliers, performance on these days is very similar to the rest of the week.
Yet, overall the spread is consistent throughout the week, suggesting our results are consistent over time, regardless of when the experiments are run.

